Affine Weyl groups and non-Abelian discrete systems: an application to the $d$-Painlev\'e equations

A non-abelian generalisation of a birational representation of affine Weyl groups and their application to the discrete dynamical systems is presented. By using this generalisation, non-commutative analogs for the discrete systems of $A_n^{(1)}$, $n \geq 2$ type and of $d$-Painlev\'e equations with an additive dynamic were derived. A coalescence cascade of the later is also discussed.

==> app3.tex <==
%\newpage
\section{Continuous limits}
\label{app:cont_lim}

As in Appendix \ref{app:deg_data}, capital letters correspond to the differential equation and $\varepsilon$ is a small parameter.

\subsection{\ref{eq:dPD4} $\to \text{\ref{eq:P5sys}}$}
\begin{gather}
    ?????
\end{gather}

\subsection{\ref{eq:dPD5'} $\to \text{\ref{eq:P40sys}}$}
\begin{gather}
    ?????
\end{gather}

\subsection{\ref{eq:dPD5} $\to \text{\ref{eq:P36sys}}$}
\begin{gather}
    ?????
\end{gather}

\subsection{$\{ \text{\ref{eq:dPD6}}, \, \text{\ref{eq:dPE6}} \} \to \text{\ref{eq:P20sys}}$}
\phantom{}
\begin{itemize}
\item[\textbullet] 
$\text{\ref{eq:dPD6}} \to \text{\ref{eq:P20sys}}$:
\begin{gather}
\begin{aligned}
    f
    &= 1 + \varepsilon \, Q + \tfrac14 \, \varepsilon^2 \, P,
    &&&
    g
    &= - 1 + \varepsilon \, Q - \tfrac14 \, \varepsilon^2 \, P,
    &&&
    t
    &= - 1 - \tfrac12 \, \varepsilon^2 \, T
    - \tfrac14 (\mathrm{A}_1 - 1) \, \varepsilon^3,
\end{aligned}
\\[1mm]
\begin{aligned}
    \beta_0
    &= - 1,
    &&&
    \beta_1
    &= 2 + \alpha_1 - \tfrac12 (\mathrm{A}_1 - 1) \, \varepsilon^2.
\end{aligned}
\end{gather}

\item[\textbullet] 
$\text{\ref{eq:dPE6}} \to \text{\ref{eq:P20sys}}$:
\begin{gather}
\begin{aligned}
    q
    &= - 1 - \varepsilon \, Q - \tfrac14 \, \varepsilon^2 \, P,
    &&&
    p
    &= 1 - \varepsilon \, Q + \tfrac14 \, \varepsilon^2 \, P,
    &&&
    t
    &= 2 + \tfrac14 (\mathrm{A}_1 - 1) \, \varepsilon^3,
\end{aligned}
\\[1mm]
\begin{aligned}
    \alpha_1
    &= - 1 - \tfrac12 \, \varepsilon^2 \, T,
    &&&
    \alpha_2
    &= 3 + \tfrac12 \, \varepsilon^2 \, T.
\end{aligned}
\end{gather}
\end{itemize}

\subsection{$\{ \text{\ref{eq:dPD6'}}, \, \text{\ref{eq:dPE6'}} \} \to \text{\ref{eq:P20sys}}$}
\phantom{}
\begin{itemize}
\item[\textbullet] 
$\text{\ref{eq:dPD6'}} \to \text{\ref{eq:P20sys}}$:
\begin{gather}
    ?????
\end{gather}

\item[\textbullet] 
$\text{\ref{eq:dPE6'}} \to \text{\ref{eq:P20sys}}$:
\begin{gather}
    ?????
\end{gather}
\end{itemize}

\subsection{$\{ \text{\ref{eq:dPD7}}, \text{\ref{eq:dPE7}} \} \to \text{\ref{eq:P1sys}}$}
\phantom{}
\begin{itemize}
\item[\textbullet] 
$\text{\ref{eq:dPD7}} \to \text{\ref{eq:P1sys}}$:
\begin{align}
    f
    &= - \tfrac12 + \varepsilon^2 \, Q - \tfrac16 \, \varepsilon^3 \, P,
    &
    g
    &= 1 - \varepsilon^2 \, Q - \tfrac13 \, \varepsilon^3 \, P,
    &
    t
    &= - 2 + \tfrac13 \, \varepsilon^4 \, T,
    &
    \alpha_1
    &= 3 - \tfrac23 \, \varepsilon^4 \, T.
\end{align}

\item[\textbullet] 
$\text{\ref{eq:dPE7}} \to \text{\ref{eq:P1sys}}$:
\begin{align}
    q
    &= 1 + \varepsilon^2 \, Q - \tfrac16 \, \varepsilon^3 \, P,
    &
    p
    &= - 2 + 2 \varepsilon^2 \, Q + \tfrac23 \, \varepsilon^3 \, P,
    &
    t
    &= - 6 + \tfrac13 \, \varepsilon^4 \, T,
    &
    \alpha_1
    &= 4 + \tfrac23 \, \varepsilon^4 \, T.
\end{align}
\end{itemize}

%\newpage

==> app4.tex <==
\subsection{Cartan matrices and root systems}
Let us fix \textit{a generalized Cartan matrix} $C = (c_{ij})_{1 \leq i, j \leq n}$, i.e. its entries are defined by
\begin{itemize}
\item[(a)] 
$c_{ii} = 2 \quad$ for any $\quad i = 1, \dots, n$,
\vspace{1mm}

\item[(b)] 
$c_{ij} \leq 0 \quad$ for $\quad i \neq j$,
\vspace{1mm}

\item[(c)] 
$c_{ij} = 0 \quad \Leftrightarrow \quad c_{ji} = 0$. 
\end{itemize}
In fact, such a Cartan matrix leads to a reflection group. Indeed, consider $n$-dimentional vector spaces $V = \spn\PoissonBrackets{\alpha_1, \dots, \alpha_n}$ and $V^* = \spn\PoissonBrackets{\alpha_1^{\vee}, \dots, \alpha_n^\vee}$. Then, the Cartan matrix $C$ defines a natural pairing calling \textit{the Killing form}:
\begin{align}
    &&
    \angleBrackets{\, \cdot \,, \cdot\,}
    &: V \times V^*
    \to \mathbb{R},
    &
    \angleBrackets{\alpha_i, \alpha_j^\vee}
    &= c_{ij}.
    &&
\end{align}
The sets $\Delta = \PoissonBrackets{\alpha_1, \dots, \alpha_n}$ and $\Delta^\vee = \PoissonBrackets{\alpha_1^{\vee}, \dots, \alpha_n^\vee}$ are called \textit{simple roots} ad \textit{simple co-roots}. The \textit{heights} $\PoissonBrackets{h_1, \dots, h_n}$ are dual to the co-roots, i.e.
\begin{align}
    \angleBrackets{
    h_i,
    \alpha_j^\vee
    }
    &= c_{ij}. 
\end{align}
The integer linear combinations are called the root lattice, co-root lattice, and weight lattice, respectively:
\begin{align}
    &&
    Q
    &= \mathbb{Z} \, \Delta,
    &
    Q^\vee
    &= \mathbb{Z} \, \Delta^{\vee},
    &
    H
    &= \mathbb{Z}\PoissonBrackets{h_1, \dots, h_n}.
    &&
\end{align}

Note that a root lattice $Q$ correspong to Cartan matrices is connected with \textit{a Dynkin diagram} $\Omega$ as follows. Each index $i$ represents a node $\alpha_i$ and each pair of indices $(i, j)$ is joined according to the rule:
\begin{itemize}
\item[(a)] 
vertices $\alpha_i$, $\alpha_j$ are joined by $n_{ij} = c_{ij} c_{ji}$ edges,
\vspace{1mm}
\item[(b)]
between each non-single edge the symbol \textgreater \, is attached towards the shorter root with respect to the Killing form $\angleBrackets{\, \cdot \,, \cdot\,}$.
\end{itemize}
In particular, for $c_{ij} c_{ji} \leq 4$ this rule can be specified as follows.
\begin{table}[H]
    \centering
    \begin{tabular}{c||c|c}
         $c_{ij} c_{ji}$
         &
         $\brackets{c_{ij}, \, c_{ji}}$
         &
         $\alpha_i
         \quad\quad\quad\,\,
         \alpha_j$
         \\
         \hline\hline
         0
         & $\phantom{\dfrac{1}{}}(0,0)\phantom{\dfrac{1}{}}$
         & \scalebox{0.8}{\input{pictures/cart_dyn/case_0.tex}}
         \\[2.5mm]
         1
         & $(-1,-1)$
         & \scalebox{0.8}{\input{pictures/cart_dyn/case_1.tex}}
         \\[2.5mm]
         2
         & $(-2,-1)$
         & \scalebox{0.8}{\input{pictures/cart_dyn/case_2.tex}}
         \\[2.5mm]
         3
         & $(-3,-1)$
         & \scalebox{0.8}{\input{pictures/cart_dyn/case_3.tex}}
         \\[2.5mm]
         4
         & $(-2,-2)$
         & \scalebox{0.8}{\input{pictures/cart_dyn/case_4_1.tex}}
         \\[2.5mm]
         4
         & $(-4,-1)$
         & \scalebox{0.8}{\input{pictures/cart_dyn/case_4_2.tex}}
    \end{tabular}
\end{table}
The root system $\Delta$ is \textit{irreducible} if the related Dynkin diagram is connected.

\subsection{Finite and affine reflection groups}
Consider a linear map $s_{\alpha_i}$ defined as
\begin{align}
    &&
    s_{\alpha_i}
    &: V \to V,
    &
    s_{\alpha_i} (\alpha_j)
    &= \alpha_j - \angleBrackets{\alpha_j, \alpha_i^\vee} \alpha_i.
    &&
\end{align}
It is called \textit{a reflection operator} and satisfies the properties:
\begin{itemize}
\item[(a)] 
$s_{\alpha_i}(\alpha_i) = - \alpha_i \quad$ for any $\quad i = 1, \dots, n$;
\vspace{1mm}

\item[(b)]
$s_{\alpha_i}^2 = 1$, i.e. they are involutions;
\vspace{1mm}

\item[(c)]
$\angleBrackets{s_{\alpha_i}(\alpha_j), s_{\alpha_i}(\alpha_k)^\vee} = \angleBrackets{\alpha_j, \alpha_k^\vee}$, i.e. they are isometries.
\end{itemize}

Let $W'$ be a group generated by $s_{\alpha_1}$, $\dots$, $s_{\alpha_n}$. Consider elements $s_1$, $\dots$, $s_n$ satisfying the relations
\begin{align}
    \label{eq:braidrel}
    &&
    (s_i \, s_j)^{m_{ij}}
    &= 1,
    &
    i
    &\neq j,
    &&
\end{align}
where $m_{ij}$ are defined by
\begin{align}
    \label{eq:crystprop}
    c_{ij} c_{ji}
    &= 4 (\cos{\brackets{\pi \, m_{ij}^{-1}}})^2
\end{align}
Relations \eqref{eq:braidrel} are \textit{braid relations}.
Hence, the exponents are defined by the value of the product $c_{ij} c_{ji}$ as below
\begin{table}[H]
    \centering
    \begin{tabular}{c||ccccc}
         $c_{ij} c_{ji}$
         & 0
         & 1
         & 2
         & 3
         & $\geq 4$
         \\
         \hline\hline
         $m_{ij}$
         & 2 
         & 3
         & 4
         & 6
         & $\infty$
    \end{tabular}
\end{table}
\begin{rem}
Conditions \eqref{eq:crystprop} are also known as \textit{the crystallographic property} that naturally arises from the definition of the Cartan matrices. 
\end{rem}

It is well-known that $W'$ is isomorphic to the affine Weyl group generated by $s_1$, $\dots$, $s_n$, since one can define an isomorphism $\eta: W \to W'$, satisfying the property
\begin{align}
    &&
    \eta (s_{i})
    &= s_{\alpha_i}
    &
    i
    &= 1, \dots, n.
    &&
\end{align}
Let us denote by $W=W(C) = \angleBrackets{s_1, \dots, s_n}$ the Weyl group defined by the generators 
$s_i$ satisfying the relations 
\begin{align}
    &&
    s_i^2
    &=1,
    &
    (s_i \, s_j)^{m_{ij}}
    &= 1,
    &
    i \neq j.
    &&
\end{align} 
The generators $s_i$ act naturally on the root lattice $Q$ by reflections 
\begin{align}
    \label{eq:refl}
    s_{i} (\alpha_j)
    &= \alpha_j
    - \angleBrackets{\alpha_j,\alpha_i^\vee} \alpha_i
    = \alpha_j - c_{ij} \alpha_i
    .
\end{align}
Note that the root system of $W$ is a subset $\Phi$ of $Q$ defined by $\Phi = W' \, \Delta$. 

For any irreducible root system $\Phi$ one can define the root 
\begin{align}
    \tilde \alpha    
    &= \sum_{1 \leq i \leq n} c_i \, \alpha_i
\end{align}
whose height is maximal. Such a root is unique and is called \textit{the highest root}. Let us extend the Cartan matrix by considering this root. By addling the column $c_{0} = (c_{0 j})$ and row $r_{0} = (c_{i 0})$ according to the rule
\begin{align}
    \label{eq:simple_root}
    &&
    c_{00}
    &= 2,
    &
    c_{0 j}
    &= \angleBrackets{- \tilde\alpha, \alpha_j^\vee},
    &
    c_{i 0}
    &= \angleBrackets{\alpha_i^\vee, - \tilde\alpha},
    &&
\end{align}
we obtain \textit{the extended Cartan matrix} $C^{(1)} = (c_{ij})_{0 \leq i, j \leq n}$ which defines the affine Weyl group $W(C^{(1)})$. The additional node $\alpha_0$ in the Dynkin diagram $\Omega$ is adjoined according to \eqref{eq:simple_root}. The corresponding vector space $V^{(1)}$ is spanned by $\Delta^{(1)} = \Delta \cup \{\alpha_0\}$ and for the reflection $s_{\alpha_0}$ we write $s_0$. Remark that the extended Cartan matrix is no longer associated to the inner product of the Euclidean space. 

\textit{An extended affine} Weyl group $\widetilde{W}^{(1)}$ is the affine Weyl group together with $\pi_{\sigma}$ such that $\pi_{\sigma} s_i = s_{\sigma{(i)}} \pi_{\sigma}$.

Here we consider an affine Weyl group $W = \angleBrackets{s_0, \dots, s_n}$ with the corresponding affine root system $\Phi^{(1)} = \PoissonBrackets{w.\Delta^{(1)} \, \big| \,w \in W}$. Introduce \textit{the null vector} $\delta$ by
\begin{align}
    &&
    \delta
    &:= \alpha_0 + \tilde \alpha,
    &
    \angleBrackets{\delta, \alpha^{\vee}}
    &= 0
    &
    \forall \, 
    \alpha^\vee
    &\in (V^{(1)})^*.
    &&
\end{align}
Let $V_0 = \PoissonBrackets{\lambda \in V \, \big| \, \angleBrackets{\lambda, \delta} = 0}$. Therefore, the $\Phi^{(1)}$ has another representation, i.e.
\begin{align}
    \Phi^{(1)}
    &= \PoissonBrackets{\alpha + \mathbb{Z} \, \delta \, \big| \, \alpha \in \Phi}.
\end{align}

An key property of the aﬃne root systems is that the associated Weyl groups are of inﬁnite order and include \textit{the translations}. Geometrically it means that the actions of $W(C^{(1)})$ as affine transformations in a hyperplane $H \subset V^{(1)}$,
\begin{align}
    H
    &= \PoissonBrackets{h \in V^{(1)} \, \big| \, \angleBrackets{h, \delta^\vee} = 1}
    ,
\end{align}
does not pass through the origin and gives rise to the translations on the hyperplane. In particular, we have
\begin{align}
    s_0 s_{\tilde \alpha} (h)
    &= s_{\delta - \tilde \alpha} s_{\tilde{\alpha}} (h)
    = h + \tilde \alpha,
\end{align}
where the actions associated with the affine root $\alpha - k \delta \in \Phi^{(1)}$ on $H$ are defined by
\begin{align}
    s_{\alpha - k \delta} (h)
    &= h - \brackets{
    \angleBrackets{h, \alpha^\vee} - k
    } \, \alpha.
\end{align}

Consider $\mu \in V_0$ such that $\angleBrackets{\mu, \mu^\vee} \neq 0$. The translation element $T_{\mu}$, or \textit{the Kac translation}, associated to $\mu \in W(C^{(1)})$ is given by $T_{\mu}:= s_{\delta - \mu} \, s_{\mu}$.
We remarks some its properties. 
\begin{itemize}
\item[(a)] 
$T_{\alpha} T_{\beta} = T_{\alpha + \beta} \quad$ for any $\quad \alpha, \beta \in V_0$.
\vspace{1mm}

\item[(b)]
$w \, T_{\mu} = T_{w(\mu)} \, w \quad$ for any $\quad w \in W$.
\vspace{1mm}

\item[(c)]
$T_{\alpha} (\beta) = \alpha - \angleBrackets{\alpha, \beta} \delta$.
\end{itemize}

==> j.tex <==
\medskip

\subsection*{Data Availibility} 
This manuscript has no associated data available.

\subsection*{Declarations}
\subsubsection*{Competing interests}
The authors declare that they have no competing interests.
